Non Common Path Aberrations Correction

The primary goal of this thesis was the correction of Non-Common-Path-Aberrations in the SPHERE instrument for helping it meeting its contrast requirements. SPHERE's purpose is the search and characterization of giant exo-planets around nearby stars. The author implemented a method called Electric Field Conjugation that he tested in simulation as well as on the real system. A full week was booked in SPHERE schedule a few days before the second commissioning in June 2014. It gave the opportunity to the author to travel to the VLT in Chile and experiment directly on the system. The contrast gain objective of another order of magnitude in a medium-sized area has successfully been reached bringing SPHERE raw speckle contrast from about $10^{-6}$ to $10^{-7}$. The algorithm has therefore proven its value and will be further investigated and hopefully automated by the SPHERE team based on the codes developed by the author. However it is important to keep in mind that Electric Field Conjugation is more effective for follow-up studies in order to improve the quality of the observations. Indeed the area for a good correction is very limited. It can't be used for exo-planets discovery unless the corrected area is made big enough but the performance will be less.

==> Bibliography.tex <==
% Bibliography

\label{app:bibliography} % Reference the bibliography elsewhere with \autoref{app:bibliography}

\manualmark
\markboth{\spacedlowsmallcaps{\bibname}}{\spacedlowsmallcaps{\bibname}} 
\refstepcounter{dummy}

\addtocontents{toc}{\protect\vspace{\beforebibskip}} % Place the bibliography slightly below the rest of the document content in the table of contents
\addcontentsline{toc}{chapter}{\tocEntry{\bibname}}

\bibliographystyle{plainnat}

\bibliography{D:/latex/EFC/bibliography/bib_EFC}
\bibliography{D:/latex/phaseDiversity/bibliography/bib_phase_diversty}

==> Bibliography_Optics.tex <==
% Bibliography

\label{app:bibliography} % Reference the bibliography elsewhere with \autoref{app:bibliography}

%\manualmark
%\markboth{\spacedlowsmallcaps{\bibname}}{\spacedlowsmallcaps{\bibname}} 
%\refstepcounter{dummy}

%\addtocontents{toc}{\protect\vspace{\beforebibskip}} % Place the bibliography slightly below the rest of the document content in the table of contents
\addcontentsline{toc}{chapter}{\tocEntry{\bibname}}

\bibliographystyle{plainnat}
%\addbibresource{D:/latex/optics_others/bibliography/bib_optics.bib}
%\printbibliography[heading=subbibliography] 


\bibliography{D:/latex/optics_others/bibliography/bib_optics}

==> Dedication.tex <==
% Dedication

\thispagestyle{empty}
\refstepcounter{dummy}

\pdfbookmark[1]{Dedication}{Dedication} % Bookmark name visible in a PDF viewer

\vspace*{3cm}

\begin{center}
\emph{Ohana} means family. \\
Family means nobody gets left behind, or forgotten. \\ \medskip
--- Lilo \& Stitch    
\end{center}

\medskip

\begin{center}
Dedicated to the loving memory of Rudolf Miede. \\ \smallskip
1939\,--\,2005
\end{center}

==> Publication.tex <==
% Publications - a page listing research articles written using content in the thesis

\pdfbookmark[1]{Publications}{Publications} % Bookmark name visible in a PDF viewer

\chapter*{Publications} % Publications page text

Some ideas and figures have appeared previously in the following publications:

\bigskip

\noindent Put your publications from the thesis here. The packages \texttt{multibib} or \texttt{bibtopic} etc. can be used to handle multiple different bibliographies in your document.

==> body_EFC_code.tex <==
\relSection{Electric Field Conjugation}

This sections describes the code related to the electric field conjugation.

Electric Field Conjugation is based on a step of calibration and a step of iterations.
The basic idea of the calibration is to poke the deformable mirror of the adaptive optics with many different modes. Then for each mode a shape (called probe) is applied to the deformable mirror which changes the speckle patterns. The changes in intensity are stored in a interaction matrix that transforms the changes caused by the probes to corresponding modes amplitudes.
When iterating one step consists on applying the probes and then using the speckles pattern changes in order to deduce the amplitudes of the modes to apply. This corresponds to the inversion of the interaction matrix.

As the interaction matrix can be measured there is no need for complicated piece of code. The only features really needed are the extraction of pixels in a specific area and then matrix reshaping. This is actually shown in the How-to tutorials section.

However one would like to simulate the process or maybe build synthetic interaction matrices and that requires functions.

\relSubsection{Code Architecture}

\relSubsubsection{Area}
Area functions are used to identified the pixels in the area of interest. They can be used on their own to reduce data once the sampling of the detector has been defined but they are also used in the modes functions in order to know how to set the frequency of the Fourier modes.

\begin{description}
\item[get\_anglePortionRing\_area] Get an area defined by a portion of a ring.
\item[get\_ESO\_area]              Get an area defined by a mask saved as a fits file.
\item[get\_rect\_hori\_area]        Get horizontally shifted rectangle(s) area.
\end{description}

\relSubsubsection{Probes}
Each function defines a set of probes.

\begin{description}
\item[hori\_probes]    Create two horizontally shifted rectangular probes.
\item[horver\_2probes] Create two L-shaped probes covering a squared ring.
\item[horver\_4probes] Create four probes (2 vertical and 2 horizontal rectangles)
\item[rot\_probes]     Create two rectangular probes shifted in inclined direction.
\item[vert\_probes]    Create two vertically shifted rectangular probes.
\end{description}

\relSubsubsection{Modes}
Each function defines a set of modes matching the wanted area. Modes commands for the DM can be saved for SPHERE application using the function saxo\_vec2ima\_volt().

\begin{description}
\item[anglePortionRing\_modes] Define Fourier modes for an portion of ring.
\item[ESO\_modes]              Define Fourier modes for an area defined by a mask.
\item[IF\_modes]               Define influence functions modes for any area types.
\item[load\_sing\_modes]        Load singular modes from file.
\item[rect\_hori\_modes]        Define Fourier modes for horizontally shifted rectangle(s)
\item[ring\_modes]             Define Fourier modes for right half or whole ring.
\item[save\_sing\_modes]        Build singular modes based on old modes.
\end{description}

\relSubsubsection{Others}
Other functions with no link with one another.

\begin{description}
\item[analize\_EFC\_results] Analize convergence of EFC iterations
\item[apply\_simu\_EFC]      Simulate sets of iterations of EFC with random speckles
\item[build\_simu\_IM]       Build a simulated Interaction Matrix for EFC.
\item[influence\_matrices]  Interpolate the influence functions and invert them.
\item[saxo\_vec2ima\_volt]   convert SAXO voltage vector to 2-D imag
\item[SPHEREfitsread]      Transform SPHERE images for matching simulations.
\end{description}


\relSubsubsection{Simulation}
Simulations of Electric Field Conjugation are described in how-to tutorials. The principle is to call a probe function, a mode function, the simulation of the interaction matrix (build\_simu\_IM()) and to finish to simulate some iterations using apply apply\_simu\_EFC{}. In order to measure the residual intensity in the area of interest one should use the function analize\_EFC\_results().

\relSubsubsection{Real data application}
The only functions used for real data application are the area functions to define the pixels to extract and the function to analyze the EFC iterations (analize\_EFC\_results()). The function SPHEREfitsread() is also used for rotating SPHERE images in a way that it fits the coordinates of the simulations.

\relSubsection{How-to tutorials}
The first tutorial to look at is howTo\_simulate\_EFC as it present the simplest possible simulation of Electric Field Conjugation. It is the better way to get a first experience with the functions. The howTo\_simulate\_EFC\_SPHERE is a more advanced script which explain how to simulate Electric Field Conjugation for SPHERE. This script can be used to test modes and to see in advance what has a chance to work or not. It uses a folder called howTo\_simulate\_EFC\_SPHERE\_outputs for saving the computed modes, probes and interaction matrices. The two last script concern the real application of Electric Field Conjugation. howTo\_build\_IM explain how to build the interaction matrix. A set of fits file is stored in the folder howTo\_build\_IM\_fits and the outputs matrices are saved in howTo\_build\_IM\_outputs. To finish howTo\_build\_IM explain how to iterate. The set of fits file for this script is stored in howTo\_iterate\_EFC\_fits. Other inputs are saved in howTo\_iterate\_EFC\_inputs and the outputs (images with iterations, correction vectors) go into howTo\_iterate\_EFC\_outputs. The last folder SPHERE\_fits includes the apodizer, the influence functions, the interaction matrix for building the slopes and the slaved actuator map of SPHERE. It is used by the simulations scripts.

\begin{description}
\item[howTo\_build\_IM]            Tutorial to build the IM from raw .fits file.
\item[howTo\_iterate\_EFC]         Tutorial for iterating EFC
\item[howTo\_simulate\_EFC]        End-to-end simulation of the EFC with ideal coro.
\item[howTo\_simulate\_EFC\_SPHERE] End-to-end simulation of the EFC with SPHERE.
\end{description}



==> body_utils_code.tex <==
\relSection{Utility functions}

This section describes the utility functions (./matlab\_reference/utils/). It includes the functions for modelling the pupil, for modelling the detector, to apply Fourier optics as well as a bunch of other random tools.

    
\relSubsection{Code Architecture}
There is no real architecture in this set of files. However we can define some types of function.

\relSubsubsection{Fourier Optics}
Key functions to model a optical system. The principle of these functions is to have only one input parameter. This parameter is in fact a structure that the user defines as he likes to create for example a coronograph or to include perturbations in the pupil. In order to define the pupil sampling please refer to the \ref{sec:pupilDef} subsection. If you want a particular sampling for the detector it is important that the sampling of the pupil match it.

\begin{description}
\item[complPupil2complFocal]    Use Fourier optics to compute focal plane from pupil
\item[complPupil2intensFocal]   Get the intensity in the focal plane from pupil.
\item[plot\_pupil\_and\_PSF]       Various pre-defined plots of pupils and PSFs.
\end{description}

\relSubsubsection{Pupil definition}
\label{sec:pupilDef}
Definition of the pupil mask and pupil sampling. It is important and not trivial to define the right sampling for the pupil when using Fast Fourier Transforms to compute the focal plane. This functions do it automatically based on a few parameters.

\begin{description}
\item[get\_pupil\_sampling]       Compute pupil sampling and mask according to parameters
\item[get\_pupil\_sampling\_no\_zp] Get pupil sampling without zero padding included.
\item[interpPupilFromModel]     Interpolate a pupil model and optionally rotate it.
\item[get\_Johann\_spiders]       Compute spiders for the AOF
\item[addSpiders]               Add a simple model of spiders into the pupil mask
\end{description}


\relSubsubsection{Detector definition}
Definition of the detector sampling.

\begin{description}
\item[get\_detector\_sampling]    Compute detector sampling according to parameters.
\item[get\_image\_area]           Get the indices of the area corresponding to an image size.
\end{description}


\relSubsubsection{Others}
Other tools not related with one another.

\begin{description}
\item[field\_exist]              Check whether or not the field fieldname exists in mystructure
\item[field\_valid]              Check if fieldname exists and is not empty in mystructure 
\item[findCentroid]             Compute the centroid of a blob in an image.
\item[get\_DFT\_matrix]           Compute the DFT matrices for a given detector and pupil.
\item[measure\_noise]            Measure the noise in an image by masking the central part.
\item[meter2rad]                Convert phase variation from meter to radian.
\item[rad2meter]                Convert phase variation from radian to nanometer.
\item[zernike2pixels]           Build the matrix to convert Zernikes into pixels value.
\end{description}


\relSubsection{How-to tutorials}
There is only one (but probably the most important of all) how-to tutorial for these codes. 

\begin{description}
\item[howTo\_complPupil2Focal] It explains how to use the functions complPupil2complFocal() and complPupil2intensFocal(). But it helps also understanding the computation of the sampling of the pupil and the detector as well as how to plot the images. The two functions are very flexible and many things can be done with them when setting the right parameters. For instance one can add perturbations in the pupil or defines a home-made coronograph.
\end{description}



